Federated Continual Learning with Weighted Inter-client Transfer

There has been a surge of interest in continual learning and federated learning, both of which are important in deep neural networks in real-world scenarios. Yet little research has been done regarding the scenario where each client learns on a sequence of tasks from a private local data stream. This problem of federated continual learning poses new challenges to continual learning, such as utilizing knowledge from other clients, while preventing interference from irrelevant knowledge. To resolve these issues, we propose a novel federated continual learning framework, Federated Weighted Inter-client Transfer (FedWeIT), which decomposes the network weights into global federated parameters and sparse task-specific parameters, and each client receives selective knowledge from other clients by taking a weighted combination of their task-specific parameters. FedWeIT minimizes interference between incompatible tasks, and also allows positive knowledge transfer across clients during learning. We validate our FedWeIT against existing federated learning and continual learning methods under varying degrees of task similarity across clients, and our model significantly outperforms them with a large reduction in the communication cost. Code is available at https://github.com/wyjeong/FedWeIT

==> main/experiments/3_resnet_wraptable.tex <==
%\vspace{0.3in}
\begin{wraptable}{r}{2.1in}
\footnotesize
\vspace{-0.1in}
\caption{\small FCL results on NonIID-50 dataset with ResNet-18.}
\label{table:resnet}
\vspace{0.05in}
\begin{tabular}{lcc} 
\hline
\multicolumn{1}{c||}{} & \multicolumn{2}{c}{\textbf{ResNet-18}} \\ \hline \hline
\multicolumn{1}{c||}{\textbf{Methods}} & \multicolumn{1}{c|}{\textbf{Acc.}} & \multicolumn{1}{c}{\textbf{Capa.}} \\ \hline
\multicolumn{1}{l||}{\textbf{Local-APD}} & \multicolumn{1}{c|}{92.44\%} & \multicolumn{1}{c}{110\%}\\
\hdashline
\multicolumn{1}{l||}{\textbf{FedProx-APD}} & \multicolumn{1}{c|}{92.89\%} & \multicolumn{1}{c}{121\%} \\
\multicolumn{1}{l||}{\textbf{FedWeIT}} & \multicolumn{1}{c|}{\textbf{94.86\%}} & \multicolumn{1}{c}{\textbf{109\%}} \\
\hline
\end{tabular}
\vspace{-0.1in}
\end{wraptable}


==> main/experiments/asyn_table.tex <==
\begin{wraptable}{rb!}{1.8in}
\footnotesize
\caption{\footnotesize Averaged performance of FedWeIT with synchronous and asynchronous federated continual learning scenario.}
\label{table:asyn}
\begin{tabular}{lc} 
\hline
\multicolumn{2}{c}{\textbf{NonIID-50}} \\ \hline \hline
\multicolumn{1}{c||}{\textbf{FedWeIT}} & \multicolumn{1}{c}{\textbf{Accuracy (\%)}}\\ \hline
\multicolumn{1}{l||}{\textbf{Synchronous}} & \multicolumn{1}{c}{\textbf{84.11 $\pm$ 0.27}} \\
\multicolumn{1}{l||}{\highlight{\textbf{Asynchronous}}} & \multicolumn{1}{c}{\textbf{84.40 $\pm$ 0.41}} \\
\hline
\end{tabular}
\end{wraptable}


==> main/experiments/main_table.tex <==
\begin{table*}[t]
\hspace{-0.5in}
\centering
\footnotesize
%\fontsize{8.5pt}{8.5pt}\selectfont
    \caption{\footnotesize
 Averaged Per-task performance on both dataset during FCL with $5$ clients (fraction=1.0). We measured task accuracy and model size after completing all learning phases over $3$ individual trials. We also measured C2S/S2C communication cost for training each task.}
    \begin{tabular}{lccccccc}
    \hline
    \hline
    \multicolumn{2}{c||}{} & \multicolumn{3}{c||}{\textbf{NonIID-50 Dataset} (\emph{F}=1.0, \emph{R}=20)} & \multicolumn{3}{c}{\textbf{Overlapped CIFAR-100} (\emph{F}=1.0, \emph{R}=20)} \\ \hline \hline
    
    \multicolumn{1}{c||}{\textbf{Methods}} & \multicolumn{1}{c||}{\textbf{FCL}} & \multicolumn{1}{c|}{\textbf{Accuracy}} & \multicolumn{1}{c|}{\textbf{Model Size}} & \multicolumn{1}{c||}{\textbf{C2S/S2C Cost}} & \multicolumn{1}{c|}{\textbf{Accuracy}} & \multicolumn{1}{c|}{\textbf{Model Size}} & \multicolumn{1}{c}{\textbf{C2S/S2C Cost}} \\ \hline
    %\multicolumn{1}{c||}{\textbf{STL}} & \multicolumn{1}{c|c|c||}{57.15 (x.xx) xxx (100\%) N/A} & \multicolumn{1}{c|}{85.78 (x.xx)} & \multicolumn{1}{c|}{xxx (100\%)}  & \multicolumn{1}{c}{N/A}\\ \hdashline
    
    %\multicolumn{1}{l||}{\textbf{STL}} & \multicolumn{1}{c|}{85.78 \tiny{\tiny{$\pm$ 0.17}}} & 
    %\multicolumn{1}{c||}{610.0 (N/A)} & 
    %\multicolumn{1}{c|}{57.15 \tiny{\tiny{$\pm$ 0.07}}} & \multicolumn{1}{c}{610.0 (N/A)}\\ \hdashline
    
    \multicolumn{1}{l||}{\textbf{Local-EWC}} & \multicolumn{1}{c||}{$\bsy\times$} & 
    \multicolumn{1}{c|}{74.30 ($\pm$ 0.08)} & 
    \multicolumn{1}{c|}{0.061 \tiny{GB}} &
    \multicolumn{1}{c||}{N/A} &
    \multicolumn{1}{c|}{44.26 ($\pm$ 0.43)} & 
    \multicolumn{1}{c|}{0.061 \tiny{GB}} &
    \multicolumn{1}{c}{N/A}\\ 

    \multicolumn{1}{l||}{\textbf{\TBDD{Stable-SGD}}} & \multicolumn{1}{c||}{$\bsy\times$} & 
    \multicolumn{1}{c|}{\TBDD{xx.xx ($\pm$ 0.xx)}} & 
    \multicolumn{1}{c|}{0.061 \tiny{GB}} &
    \multicolumn{1}{c||}{N/A} &
    \multicolumn{1}{c|}{\TBDD{xx.xx ($\pm$ 0.xx)}} & 
    \multicolumn{1}{c|}{0.061 \tiny{GB}} &
    \multicolumn{1}{c}{N/A}\\ 
    
    
    \multicolumn{1}{l||}{\textbf{Local-APD}} & \multicolumn{1}{c||}{$\bsy\times$} & 
    \multicolumn{1}{c|}{81.42 ($\pm$ 0.72)} & 
    \multicolumn{1}{c|}{0.090 \tiny{GB}} &
    \multicolumn{1}{c||}{N/A} &
    \multicolumn{1}{c|}{50.82 ($\pm$ 0.33)} & 
    \multicolumn{1}{c|}{0.073 \tiny{GB}} &
    \multicolumn{1}{c}{N/A}\\ 
    \hdashline
    
    \multicolumn{1}{l||}{\textbf{FedProx}} & \multicolumn{1}{c||}{$\checkmark$} & 
    \multicolumn{1}{c|}{63.69 ($\pm$ 1.75)} & 
    \multicolumn{1}{c|}{0.061 \tiny{GB}} &
    \multicolumn{1}{c||}{1.22 / 1.22 \tiny{GB}} &
    \multicolumn{1}{c|}{33.83 ($\pm$ 0.48)} &
    \multicolumn{1}{c|}{0.061 \tiny{GB}} &
    \multicolumn{1}{c}{1.22 / 1.22 \tiny{GB}}\\ 
    
    \multicolumn{1}{l||}{\textbf{Scaffold}} & \multicolumn{1}{c||}{$\checkmark$} & 
    \multicolumn{1}{c|}{30.84 ($\pm$ 1.41)} & 
    \multicolumn{1}{c|}{0.061 \tiny{GB}} &
    \multicolumn{1}{c||}{2.44 / 2.44 \tiny{GB}} &
    \multicolumn{1}{c|}{22.80 ($\pm$ 0.47)} &
    \multicolumn{1}{c|}{0.061 \tiny{GB}} &
    \multicolumn{1}{c}{2.44 / 2.44 \tiny{GB}}\\ 
    
    \multicolumn{1}{l||}{\textbf{FedCurv}} & \multicolumn{1}{c||}{$\checkmark$} & 
    \multicolumn{1}{c|}{72.39 ($\pm$ 0.32)} & 
    \multicolumn{1}{c|}{0.061 \tiny{GB}} &
    \multicolumn{1}{c||}{1.22 / 1.22 \tiny{GB}} &
    \multicolumn{1}{c|}{40.36 ($\pm$ 0.44)} &
    \multicolumn{1}{c|}{0.061 \tiny{GB}} &
    \multicolumn{1}{c}{1.22 / 1.22 \tiny{GB}}\\ 
    
    \multicolumn{1}{l||}{\textbf{FedProx-EWC}} & \multicolumn{1}{c||}{$\checkmark$} & 
    \multicolumn{1}{c|}{68.18 ($\pm$ 0.58)} & 
    \multicolumn{1}{c|}{0.061 \tiny{GB}} &
    \multicolumn{1}{c||}{1.22 / 1.22 \tiny{GB}} &
    \multicolumn{1}{c|}{41.91 ($\pm$ 0.47)} &
    \multicolumn{1}{c|}{0.061 \tiny{GB}} &
    \multicolumn{1}{c}{1.22 / 1.22 \tiny{GB}}\\ 

    \multicolumn{1}{l||}{\textbf{\TBDD{FedProx-SSGD}}} & \multicolumn{1}{c||}{$\checkmark$} & 
    \multicolumn{1}{c|}{\TBDD{76.55 ($\pm$ 0.xx)}} & 
    \multicolumn{1}{c|}{0.061 \tiny{GB}} &
    \multicolumn{1}{c||}{1.22 / 1.22 \tiny{GB}} &
    \multicolumn{1}{c|}{\TBDD{43.29 ($\pm$ 1.45)}} &
    \multicolumn{1}{c|}{0.061 \tiny{GB}} &
    \multicolumn{1}{c}{1.22 / 1.22 \tiny{GB}}\\ 
    
    \multicolumn{1}{l||}{\textbf{FedProx-APD}} & \multicolumn{1}{c||}{$\checkmark$} & 
    \multicolumn{1}{c|}{81.20 ($\pm$ 1.24)} & 
    \multicolumn{1}{c|}{0.079 \tiny{GB}} &
    \multicolumn{1}{c||}{1.22 / 1.22 \tiny{GB}} &
    \multicolumn{1}{c|}{52.20 ($\pm$ 0.41)} &
    \multicolumn{1}{c|}{0.075 \tiny{GB}} &
    \multicolumn{1}{c}{1.22 / 1.22 \tiny{GB}}\\ 
    
    \multicolumn{1}{l||}{\textbf{\highlight{FedWeIT}}} & \multicolumn{1}{c||}{$\checkmark$} & \multicolumn{1}{c|}{\textbf{84.11 ($\pm$ 0.27)}} & 
    \multicolumn{1}{c|}{0.078 \tiny{GB}} &
    \multicolumn{1}{c||}{\textbf{0.37 / 1.07 \tiny{GB}}} &
    \multicolumn{1}{c|}{\textbf{55.16 ($\pm$ 0.19)}} &
    \multicolumn{1}{c|}{0.075 \tiny{GB}} &
    \multicolumn{1}{c}{\textbf{0.37 / 1.07 \tiny{GB}}}\\ 
    \multicolumn{1}{l||}{\textbf{\highlight{FedWeIT-V2}}} & \multicolumn{1}{c||}{$\checkmark$} & \multicolumn{1}{c|}{\textbf{xx.x ($\pm$ 0.xx)}} & 
    \multicolumn{1}{c|}{0.0xx \tiny{GB}} &
    \multicolumn{1}{c||}{\textbf{0.xx / 1.07 \tiny{GB}}} &
    \multicolumn{1}{c|}{\textbf{xx.xx ($\pm$ 0.xx)}} &
    \multicolumn{1}{c|}{0.0xx \tiny{GB}} &
    \multicolumn{1}{c}{\textbf{0.xx / 0.0x \tiny{GB}}}\\ 
    \hline\hline
    \multicolumn{1}{l||}{\textbf{Single Task}} & \multicolumn{1}{c||}{$\bsy\times$} & 
    \multicolumn{1}{c|}{85.78 ($\pm$ 0.17)} & 
    \multicolumn{1}{c|}{0.610 \tiny{GB}} &
    \multicolumn{1}{c||}{N/A} &
    \multicolumn{1}{c|}{57.15 ($\pm$ 0.07)} & 
    \multicolumn{1}{c|}{0.610 \tiny{GB}} &
    \multicolumn{1}{c}{N/A}\\
    \hline
    \hline
    \end{tabular}
    \vspace{-0.2in}
    \label{table:main}
\end{table*}

